GeoCamera: Telling Stories in Geographic Visualizations with Camera Movements

In geographic data videos, camera movements are frequently used and combined to present information from multiple perspectives. However, creating and editing camera movements requires significant time and professional skills. This work aims to lower the barrier of crafting diverse camera movements for geographic data videos. First, we analyze a corpus of 66 geographic data videos and derive a design space of camera movements with a dimension for geospatial targets and one for narrative purposes. Based on the design space, we propose a set of adaptive camera shots and further develop an interactive tool called GeoCamera. This interactive tool allows users to flexibly design camera movements for geographic visualizations. We verify the expressiveness of our tool through case studies and evaluate its usability with a user study. The participants find that the tool facilitates the design of camera movements.

==> figures/ui.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.98\textwidth]{images/interface.png}
    \caption{The user interface of \tool: (A) previewer of camera movements in the geographic visualization with geospatial targets selection, (B) a library of camera movements classified by narrative purposes, (C) camera and visual configurations and crafted examples, and (D) a location-camera hierarchical timeline.}
    % \Description{A system interface.}
    \label{fig:ui}
\end{figure*}




==> sections/3-deisng-objectives.tex <==
% \section{Design Objectives}
% \label{sec:design-objetives}
% Our research is motivated by the goal of designing an authoring tool to simplify the process of crafting geographic data videos for the general users. 
% \reviewer{(R3): To me, it would make more sense to be basing the design considerations on the information gathered in section 4 rather than relying on potentially ungrounded conjecture.}

%\subsection{Usage Scenario}
% \user is a data analyst working for a consulting company.
% She routinely conducts exploratory data analyses and reports findings to her clients.
% This time, she analyzes branch performance for a fast food brand in a large city.
% She visualizes the sales of the branches on a map and gains many insights.
% For instance, a branch with a special marketing strategy attains the highest sales in the neighborhood.
% The sales are generally low alongside a river and high in the industrial district.
% \user decides to present her findings in a video to engage the clients and explain the findings better.

% In \tool, \user uploads the sales data and visualizes the data with a 2.5D bar chart on the map.
% To give an overview, she first adjusts the map zoom to show the entire city.
% Then, she selects the highest bar in the map that represents the best-performing branch and chooses the ``Emphasizing a target'' narrative purpose  from the left sidebar of GeoCamera.
% GeoCamera automatically adds a scene to the video timeline, which employs the ``push in'' camera shot to zoom into the branch's location, highlighting this outlier in the sales data.
% Thereafter, Zoey moves the map to the riverside region and chooses the ``Making a comparison'' purpose.
% To compare the sales in this region with those in the industrial district, she changes the presentation mode to ``side-by-side'' and adds the industrial district as the comparison target.
% Hence, GeoCamera creates a scene where the camera first flies to the riverside region with the ``pan'' camera shot and then splits into two views, showing the riverside region and the industrial district simultaneously.
% Similarly, Zoey authors other scenes with GeoCamera to explain the rest of the insights she discovered.
% Finally, she adds the descriptions of these insights to each scene as subtitles and fine-tunes the duration of each scene to make the video more coherent.
% Although \user receives little training in video-making, she manages to produce an appealing geographic data video which smoothly explains and transitions between different insights with \tool.

% fixes the focus on the highest bar and neighboring regions to demonstrate the outlier. 
% She selects a camera effect, push-in, from the category of ``emphasizing a target''.
% Similarly, she connects all the story pieces with certain camera effects and produces a compelling geographic data video.



% \textbf{(C4) Modular authoring.}
% % graphics parameters, clips
% We strive to ease the creation process of geographic data videos, especially flexible customization of every camera movements used for geospatial targets.
% Since camera serves geospatial targets in single modes or in combinations, we use a modular architecture in accordance with DataClips~\cite{amini2017dataclips}.
% we first create clips of geospatial targets, then bind a set of camera movements with a clip, and assemble clips into a complete data video at last. 
% This modular authoring method enables users authoring sets of camera movements shooting at the same geospatial targets and modify narration both locally and globally with clips. 


% In this section, we first introduce two motivating scenarios for using the tool.
% Then we summarize a series of design considerations of an authoring tool for camera movements in geographic data videos.
% After that, We formulate the pipeline and describe the interaction design of the tool.

% Aforementioned findings have concluded common patterns of narrative tactics and geospatial targets of camera movements geographic data videos. 


% Based on the aforementioned motivation and design consideration, we implement \tool using collected design patterns of camera movements.
% Our main goal is to reduce human efforts in crafting camera movements in geospatial data videos.
% In this section, we first formulate the workflow of our authoring tool \tool step by step.
% Then we describe the design of \tool for camera movements schedule and visual effects configuration.

